Structured Dialogue System for Mental Health: An LLM Chatbot Leveraging the PM+ Guidelines

The Structured Dialogue System, referred to as SuDoSys, is an innovative Large Language Model (LLM)-based chatbot designed to provide psychological counseling. SuDoSys leverages the World Health Organization (WHO)'s Problem Management Plus (PM+) guidelines to deliver stage-aware multi-turn dialogues. Existing methods for employing an LLM in multi-turn psychological counseling typically involve direct fine-tuning using generated dialogues, often neglecting the dynamic stage shifts of counseling sessions. Unlike previous approaches, SuDoSys considers the different stages of counseling and stores essential information throughout the counseling process, ensuring coherent and directed conversations. The system employs an LLM, a stage-aware instruction generator, a response unpacker, a topic database, and a stage controller to maintain dialogue flow. In addition, we propose a novel technique that simulates counseling clients to interact with the evaluated system and evaluate its performance automatically. When assessed using both objective and subjective evaluations, SuDoSys demonstrates its effectiveness in generating logically coherent responses. The system's code and program scripts for evaluation are open-sourced.

==> 2.related-work.tex <==
\section{Related Work}
Nowadays it's increasingly popular to use LLMs to provide mental health care\cite{hua2024largelanguagemodelsmental}, especially in psychological counselling. However, due to lack of computing resources, most of the LLMs that showed great capability in following human instructions are only trained to serve general purposes thus behave poorly when directly used for psychological counselling. To this end, two mainstreams (categorized by whether gradient-descent-training is conducted) are developed to solve this issue: Instruction Fine-Tuning (IFT) and Chain-of-Thought Prompting (CoT)\cite{cot}.

For IFT methods, single-turn or multi-turn counselling dialogues are used to fine-tune a pre-trained LLM. ExTES-LLaMA\cite{extes}, MEChat\cite{smile}, SoulChat\cite{soulchat}, CPsyCounX\cite{CPsyCoun} are such LLMs fine-tuned on generated multi-turn dialogues. PsyChat\cite{Psychat} is a dialogue system fine-tuned on dialogues with counselor's strategy and user's behavior labelled by human.
% CBT-LLM\cite{cbt-llm} used principles of CBT to generate single-turn QA dataset which is also available for fine-tuning. 

By inducing the LLM to think and reply step by step, CoT methods like Chain of Empathy \cite{ChainOfEmpathy} and Dynamic Strategy Chain\cite{DynamicStrategyChain} enable LLMs to generate single-turn responses that are in-depth.

The challenge of multi-turn IFT methods lies in that the model fails to perceive the stage of the chatting and is unaware of the ultimate target of the counselling. Also the average turns of each training dialogue is about 8-10 in existing studies \cite{CPsyCoun,extes,smile}, indicating fine-tuned model's inability for handling longer contexts. While CoT methods fail to be applied to multi-turn dialogues.

To this end, we propose incorporating CoT into a multi-turn dialogue system to make a stage-aware psychological counselling chatbot. To the best of our knowledge, this is the first work to leverage the CoT method into multi-turn psychological counselling.


% Nowadays it's increasingly popular to use LLMs to provide mental health care\cite{hua2024largelanguagemodelsmental}, especially in psychological counselling. However, due to lack of computing resources, most of the LLMs that showed great capability in following human instructions are only trained to serve general purposes thus behave poorly when directly used for psychological counselling. To this end, two mainstreams (categorized by whether gradient-descent-training is conducted) are developed to solve this issue: Instruction Fine-Tuning (IFT) and Chain-of-Thought Prompting (CoT)\cite{cot}.

% For IFT methods, single-turn or multi-turn counselling dialogues are used to fine-tune a pre-trained LLM. To get good fine-tuning results, researchers mainly focus on the way to acquire high-quality counselling dialogue data. PsyChat\cite{Psychat} is an dialogue system fine-tuned on dialogues with counselor's strategy and user's behavior labelled by human. Zheng et al.\cite{extes} used ChatGPT to do self-talk and generated multi-turn counselling dialogues that are further used for fine-tuning. CPsyCounD\cite{CPsyCoun} is a multi-turn counseling dialogue dataset reconstructed from psychological counseling reports. SMILE\cite{smile} and SoulChat\cite{soulchat} expanded single-turn dataset to multi-turn empathetic conversations. CBT-LLM\cite{cbt-llm} used principles of CBT to generate single-turn QA dataset which is also available for fine-tuning. 

% By inducing the LLM to think and reply step by step, CoT methods enable LLMs to provide mental health support without the help of gradient descent training. Chain of Empathy \cite{ChainOfEmpathy} uses CoT prompting to incorporate psycho-therapeutic models like CBT into one response. Likewise, Dynamic Strategy Chain\cite{DynamicStrategyChain} let ChatGPT format a response under the guidance of the strategy chain. The reasoning process of CoT methods gives them the chance to generate in-depth responses. However, all CoT methods aim at generating single-turn responses.

% The challenge of multi-turn IFT methods lies in that the model fails to perceive the stage of the chatting and is unaware of the ultimate target of the counselling. Also the average turns of each training dialogue is about 8-10 in existing studies \cite{CPsyCoun,extes,smile}, indicating fine-tuned model's inability for handling longer contexts. While the flaw of all single-turn dialogue systems (regardless of IFT or CoT) is that they fail to meet the nature of psychological counselling. To be specific, in single-turn dialogue, the counselor is unable to induce the user to fully express himself/herself and the user may also feel frustrated reading large-length responses.

% To this end, we propose incorporating CoT into a multi-turn dialogue system to make a stage-aware psychological counselling chatbot. To the best of our knowledge, this is the first work to leverage the CoT method into multi-turn psychological counselling.
